Listening between the Lines: Learning Personal Attributes from Conversations

Open-domain dialogue agents must be able to converse about many topics while incorporating knowledge about the user into the conversation. In this work we address the acquisition of such knowledge, for personalization in downstream Web applications, by extracting personal attributes from conversations. This problem is more challenging than the established task of information extraction from scientific publications or Wikipedia articles, because dialogues often give merely implicit cues about the speaker. We propose methods for inferring personal attributes, such as profession, age or family status, from conversations using deep learning. Specifically, we propose several Hidden Attribute Models, which are neural networks leveraging attention mechanisms and embeddings. Our methods are trained on a per-predicate basis to output rankings of object values for a given subject-predicate combination (e.g., ranking the doctor and nurse professions high when speakers talk about patients, emergency rooms, etc). Experiments with various conversational texts including Reddit discussions, movie scripts and a collection of crowdsourced personal dialogues demonstrate the viability of our methods and their superior performance compared to state-of-the-art baselines.

==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#
# $Id: 
#

.SUFFIXES:
.SUFFIXES: .ps .dvi .tex

TEXINPUTS := .:${TEXINPUTS}
BIBINPUTS := .:${TEXINPUTS}

#all: eps dvi ps pdf # res
all: pdf
eps: fig obj

PAPER=main

LATEX=pdflatex

ps:  $(PAPER).ps

pdf: $(PAPER).pdf
dvi: $(PAPER).dvi

obj: $(patsubst %.obj, %.eps, $(wildcard *.obj))
fig: $(patsubst %.fig, %.eps, $(wildcard *.fig))

res:
	make -C results
	make -C figs

clean:
	$(RM) *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

distclean: clean
	$(RM) $(patsubst %.fig, %.eps, $(wildcard *.fig))
	$(RM) $(patsubst %.obj, %.eps, $(wildcard *.obj))

%.pdf: $(wildcard *.tex) $(wildcard *.bib)
	$(LATEX) $*
	bibtex $*
	$(LATEX) $*
	if [ -e $*.toc ] ; then $(LATEX) $* ; fi
	if [ -e $*.bbl ] ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi

%.ps: %.dvi
	dvips -Ppdf -G0 -tletter -o $@ $<
%.ps.gz: %.ps
	gzip -v9 $<

%.eps: %.obj
	tgif -print -eps $*

%.eps: %.fig
	fig2dev -L eps $< $@


==> sections/table.tex <==
\begin{appendices}
\begin{table*}[]
\begin{tabular}{ll}
\multicolumn{1}{l|}{movie -\textgreater movie}                                                                                                                                             & reddit -\textgreater movie                                                                                                                                                                \\ \hline
\multicolumn{2}{l}{correct label: astronaut}                                                                                                                                                                                                                                                                                                                                           \\
prediction: astronaut                                                                                                                                                                      & prediction: astronaut                                                                                                                                                                     \\ \hline
\multicolumn{2}{l}{correct label: salesperson}                                                                                                                                                                                                                                                                                                                                         \\
prediction: clerk                                                                                                                                                                         & prediction: banker                                                                                                                                                                        \\ \hline
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}correct label: businessperson\\ utterance: ahm... the film's great... and i just wondered -- whether you ever thought of having more... horses in it?\end{tabular}}                                                                                                                                                                      \\
\begin{tabular}[c]{@{}l@{}}prediction: director\\ utterance score: 0.05402\end{tabular}                                                                                                    & \begin{tabular}[c]{@{}l@{}}prediction: clerk\\ utterance score: 0.01360\end{tabular}                                                                                                      \\ \hline
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}correct label: monarch\\ utterance: "  first tell me are you my little volga boatman?  well... two million readers... \\"lovely little princess plays with rasputin's beard.""  a couple of bloodhounds and we have uncle tom's cabin"\end{tabular}}                                                                                       \\
\begin{tabular}[c]{@{}l@{}}prediction: monarch\\ word weights:\\ 0,0729	readers\\ 0,0729	uncle\\ 0,0729	boatman\\ 0,0729	princess\\ 0,0729	bloodhounds\\ 0,0729	toms\end{tabular}          & \begin{tabular}[c]{@{}l@{}}prediction: stewardess\\ word weights:\\ \\ 0,0305	uncle\\ 0,0397	lovely\\ 0,0818	bars\\ 0,0819	boatman\\ 0,0819	toms\\ 0,0819	cabin\end{tabular}              \\ \hline
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}correct label: scientist\\ utterance: what do you deliver on all those charters you...?  can't this thing go any faster?  come on hoagie....\end{tabular}}                                                                                                                                                                               \\
\begin{tabular}[c]{@{}l@{}}prediction: stewardess\\ word weights:\\ 0,0913	deliver\\ 0,0913	thing\\ 0,0913	go\\ 0,0913	faster\\ 0,0913	come\\ 0,1126	hoagie\\ 0,2482	charters\end{tabular} & \begin{tabular}[c]{@{}l@{}}prediction: sportsman\\ word weights:\\ 0,1090	deliver\\ 0,1090	go\\ 0,1090	faster\\ 0,1090	come\\ 0,1090	thing\\ 0,1090	charters\\ 0,1280	hoagie\end{tabular}
\end{tabular}
\caption{Example 1: although the model trained on Reddit does not have the label of astronaut, it makes a sensible prediction that it can be a scientist \\
Example 2: Both models make mistakes, however these three professions are very close in meaning and vocabulary \\
Example 3: When the occupation "director" is predicted, the utterance containing the word "film" gets 5 times greater attention\\
Example 4: When "monarch" is predicted, the word "princess" gets high score, but in the same utterance the word "cabin" is top when "stewardess" is predicted \\
Example 5: For the prediction "stewardess" the word "cabin" gets top weight, but not for "sportsman"}
\end{table*}
\end{appendices}
